Technical Report for ICCV 2023 Visual Continual Learning Challenge: Continuous Test-time Adaptation for Semantic Segmentation

The goal of the challenge is to develop a test-time adaptation (TTA) method, which could adapt the model to gradually changing domains in video sequences for semantic segmentation task. It is based on a synthetic driving video dataset - SHIFT. The source model is trained on images taken during daytime in clear weather. Domain changes at test-time are mainly caused by varying weather conditions and times of day. The TTA methods are evaluated in each image sequence (video) separately, meaning the model is reset to the source model state before the next sequence. Images come one by one and a prediction has to be made at the arrival of each frame. Each sequence is composed of 401 images and starts with the source domain, then gradually drifts to a different one (changing weather or time of day) until the middle of the sequence. In the second half of the sequence, the domain gradually shifts back to the source one. Ground truth data is available only for the validation split of the SHIFT dataset, in which there are only six sequences that start and end with the source domain. We conduct an analysis specifically on those sequences. Ground truth data for test split, on which the developed TTA methods are evaluated for leader board ranking, are not publicly available. The proposed solution secured a 3rd place in a challenge and received an innovation award. Contrary to the solutions that scored better, we did not use any external pretrained models or specialized data augmentations, to keep the solutions as general as possible. We have focused on analyzing the distributional shift and developing a method that could adapt to changing data dynamics and generalize across different scenarios.

==> detection.tex <==
% \documentclass[10pt, twocolumn, letterpaper]{article}

% \usepackage{iccv}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}

% \usepackage{multirow}
% \usepackage{xcolor}
% \usepackage{wrapfig}
% \usepackage{booktabs}
% \usepackage{times}
% \usepackage{makecell}
% \usepackage{authblk}
% \usepackage{float}


% \usepackage[breaklinks=true,bookmarks=false]{hyperref}

% \iccvfinalcopy

% % \def\iccvPaperID{30} % *** Enter the ICCV Paper ID here
% % \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% \title{SHIFT Challenge ICCV 2023 - Continuous Test-time Adaptation \\
% for Object Detection}
% % - Technical Report}

% \newcommand\todo[1]{{\color{red} [\bf TODO: #1]}}
% \newcommand{\ds}[1]{{\color{magenta} {(\bf DS:} #1)}}
% \newcommand{\bt}[1]{{\color{teal} {\bf BT:} #1}}
% \newcommand{\SC}[1]{{\color{blue} {\bf SC:} #1}}

% \newcommand{\etalcite}[2]{#1~et~al.~\cite{#2}}

% % Allow affiliations side by side
% \makeatletter
% \renewcommand\AB@affilsepx{, \protect\Affilfont}
% \makeatother
% % \setlength{\affilsep}{-0.15cm}

% \begin{document}

% \author[1,2]{Yuyang~Liu}
% \author[3,4]{Damian~Sójka}
% \author[5,6]{Dipam~Goswami}
% \author[4,7]{Sebastian~Cygert}
% \author[4,5,6]{Bartłomiej~Twardowski}
% \author[5,6]{Joost~van~de~Weijer}

% \affil[1]{Shenyang~Institute~of~Automation}
% \affil[2]{Chinese~Academy~of~Sciences}
% \affil[3]{Poznań~University~of~Technology}
% \affil[4]{IDEAS~NCBR}
% \affil[5]{Computer~Vision~Center}
% \affil[6]{Autonomous~University~of~Barcelona}
% \affil[7]{Gdańsk~University~of~Technology}

% \maketitle
% \ificcvfinal\thispagestyle{empty}\fi

\section{Object Detection}

\subsection{Motivation}
Existing  TTA algorithms frequently fine-tune the target model during testing, potentially causing overfitting in the target domain and thus a decline in the generalization of the source model, resulting in error accumulation. To address this challenge, we focus on 
% our motivation is centered on 
achieving an adaptive test-time strategy for the target model based on the mean entropy of predictions in object detection. Since entropy of predictions is a good metric to measure the degree of domain shift at test-time, we propose a method that dynamically adjusts the target model's behavior during testing based on the difference of mean entropy of the predictions between consecutive frames. 
% Our approach is rooted in monitoring the differences in mean entropy between consecutive frames. 
The objective is to continuously minimize entropy, enhancing the model's adaptability to evolving testing conditions while avoiding overfitting to individual domains.

\subsection{Our method}
We analyze the six sequences from the validation set which start and end with the source domain of clear daytime conditions and observe that the mean entropy of predictions increases for the frames having a shift in conditions to night-time or weather conditions (rainy or foggy). 
Therefore, we use a threshold on the mean entropy difference between two consecutive frames for updating the target model. When the mean entropy difference during testing is lower than this threshold, the source model maintains minimal average entropy on the test set, ensuring strong predictive performance. Thus, we focus on those frames which has a high mean entropy of predictions and thus needs adaptation.

% Observing variations in mean entropy among sequences under specific conditions (attribute=dict(weather\_coarse='clear', timeofday\_coarse='daytime')) in the validation set, we noted a sudden increase in mean entropy starting from a certain frame, signifying environmental changes. 


Our approach adapts the target model dynamically in a non-parametric manner using the mean entropy of each video frame. This approach preserves the robustness of the source model while effectively mitigating the problem of error accumulation. We compute the mean entropy generated by predictions of scores, labels, and bounding boxes, and utilize it for model optimization, resulting in a more robust representation.

Specifically, to accommodate frames with higher mean entropy, we employ an enhanced version of CoTTA~\cite{COTTA} algorithm, which utilizes knowledge distillation for adaptation and involves both a teacher model and a student model. The teacher model initially performs multiple data augmentations on the images and makes predictions. Then, based on the comparison between the average scores and a threshold value, frames are categorized into two classes: those close to the source domain and those distant from the source domain, generating pseudo-labels accordingly. The student model updates using a cross-entropy loss function with the pseudo-labels provided by the teacher model. The teacher model is updated immediately using exponential moving average (EMA) after each student model update. Furthermore, similar to CoTTA, a portion of the source model's parameters is randomly restored to alleviate catastrophic forgetting. To summarize, we update the model using the enhanced CoTTA method only for those frames having a high entropy shift from the previous frame, while keeping the model unchanged in the rest of the frames where adaptation is not essential.

\input{tables/detection_test_results}


\subsection{Experiments}
\subsubsection{Evaluation Metrics}
The evaluation metrics are defined as follows:
\begin{itemize}
    \item $mAP$ (Mean Average Precision): This metric represents the combined predictions and ground truths from all frames, offering a holistic view of the model's overall performance.
    \item $mAP_{source}$: Calculated based on the combined predictions and ground truths from the initial 0-20 frames, reflecting the model's performance in the source domain.
    \item $mAP_{target}$: Measured using the combined predictions and ground truths from frames 180-220, indicating the model's performance in the target domain.
    \item $mAP_{loop-back}$: This metric accounts for the combined predictions and ground truths from frames 380-400, providing insights into the model's adaptability in the loop-back adaptation scenario.
    \item $mAP_{drop}$: It highlights the adaptation challenges when transitioning from the source to the target domain and can be defined as: $mAP_{drop} = mAP_{source}-mAP_{target}$
    \item $overall$: This composite metric captures the overall performance: $overall = mAP-2 \times mAP_{drop}$. It provides a balanced assessment of adaptation effectiveness while considering the potential domain shift.
\end{itemize}



\subsubsection{Implementation Details}
To establish a threshold for the mean entropy difference between frames within a video sequence, we conducted statistical analysis on the validation set, which indicated that an mean entropy difference threshold of 0.01 is suitable. Consequently, during implementation, we selected frames with an mean entropy difference greater than 0.01 between consecutive frames and applied the enhanced CoTTA algorithm to adapt to the current test set.
When the mean entropy difference between consecutive frames was greater than or equal to 0.01, we reset the target model to the source model's parameters and set the model in training mode.
% model.requires\_grad\_(True) and model.train(True). 
The enhanced CoTTA algorithm employed a learning rate of 0.00025 and included three different types of data augmentations.
% , and applied paramwise\_cfg={}.
This approach allowed us to dynamically adjust the target model based on the observed changes in mean entropy, ensuring adaptability to varying conditions in the testing phase. By resetting the model when necessary, we effectively maintained model performance and minimized the risk of error accumulation.

\subsubsection{Results}
We provide a comprehensive analysis of the results obtained from our experiments, comparing the performance of different adaptation methods, including No-adaptation, CoTTA~\cite{COTTA}, and our proposed method.

As shown in Table~\ref{tab:det_res}, our proposed method achieved an $mAP$ of 39.84, showcasing competitive performance across various scenarios. Notably, it outperformed the baseline and CoTTA methods in the target domain, with an $mAP_{target}$ of 35.43. Furthermore, it exhibited superior performance in the loop-back adaptation scenario ($mAP_{loop-back}$: 49.49), indicating its adaptability. Note that the changes in $mAP_{source}$, $mAP_{target}$ and $mAP_{loop-back}$ metrics are for a small range of frames, hence reflects the performance of the model in some specific frames of the sequences. The mAP improvement of 0.21 over CoTTA suggests better performance across all frames of the sequences.

In the overall assessment, Ours demonstrated the highest overall mAP among the three methods, with an $overall$ score of 28.62. This indicates its effectiveness in achieving continuous adaptation while mitigating the impact of domain shift, as reflected in the $mAP_{drop}$ metric.

% \subsubsection{Ablation Study}

%These results highlight the advantages of our proposed method in addressing object detection challenges in evolving domains, emphasizing its potential for real-world applications.





% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{bibliography}
% }

% \end{document}

==> tables/detection_test_results.tex <==
\begin{table*}[ht]
\centering\label{tab:det_res}
\caption{Performance of our method and comparison with baselines from the server evaluation on the test split.}
\vspace{5pt}
\scalebox{1.0}{\begin{tabular}{c|cccccc}
\hline
Method        & mAP   & mAP\_source & mAP\_target & mAP\_loop\_back & mAP\_drop & overall \\ \hline
No-adaptation & 38.81 & 41.04       & 33.71       & 48.66           & 7.33      & 24.15   \\
CoTTA~\cite{COTTA}          & 39.63 & 42.75       & 34.74       & 51.16           & 8.01         & 23.63   \\
Ours          & 39.84 & 41.04       & 35.43       & 49.49           & 5.61      & 28.62   \\ \hline
\end{tabular}}
\end{table*}

==> tables/dynamic_bn.tex <==
\begin{table}[h!]
\centering
\caption{\ds{maybe show shortened version of param search for dynamic BN and LR}.}
\label{tab:dynamic_bn}
\scalebox{1.0}{
\begin{tabular}{cc|cc}
\hline

% \multicolumn{3}{c}{Adapted Weights} & \multirow{2}{*}{mIoU} \\ \hline
Dynamic BN statistics & Learning rate & $mIoU$ & $overall$ \\ \hline

& 0.00006/8 & 58.6 & 42.1 \\
\checkmark & 0.00006/8 & \textbf{58.8} & 47.3 \\
\checkmark & 0.00006/4 & 58.6 & \textbf{49.1} \\

\hline
\end{tabular}}
\end{table}

==> tables/pixel_filtering.tex <==
\begin{table}[h!]
\centering
\caption{\ds{maybe show shortened version of param search for entropy threshold}.}
\label{tab:pixel_filtering}
\scalebox{1.0}{
\begin{tabular}{cc|cc}
\hline

Pixel Filtering & $mIoU$ & $overall$ \\ \hline

 & 58.6 & 49.1 \\
\checkmark & 58.8 & \textbf{50.2} \\

\hline
\end{tabular}}
\end{table}
